Studying Behavioral Addiction by Combining Surveys and Digital Traces: A Case Study of TikTok

Opaque algorithms disseminate and mediate the content that users consume on online social media platforms. This algorithmic mediation serves users with contents of their liking, on the other hand, it may cause several inadvertent risks to society at scale. While some of these risks, e.g., filter bubbles or dissemination of hateful content, are well studied in the community, behavioral addiction, designated by the Digital Services Act (DSA) as a potential systemic risk, has been understudied. In this work, we aim to study if one can effectively diagnose behavioral addiction using digital data traces from social media platforms. Focusing on the TikTok short-format video platform as a case study, we employ a novel mixed methodology of combining survey responses with data donations of behavioral traces. We survey 1590 TikTok users and stratify them into three addiction groups (i.e., less/moderately/highly likely addicted). Then, we obtain data donations from 107 surveyed participants. By analyzing users' data we find that, among others, highly likely addicted users spend more time watching TikTok videos and keep coming back to TikTok throughout the day, indicating a compulsion to use the platform. Finally, by using basic user engagement features, we train classifier models to identify highly likely addicted users with $F_1 \geq 0.55$. The performance of the classifier models suggests predicting addictive users solely based on their usage is rather difficult.

==> tab-latex/characterization.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lp{6.5cm} rlll}
    \toprule
    Concept & Definition & Calculation & \multicolumn{3}{c}{Significance} \\ \midrule
    & \multicolumn{5}{c}{\textbf{Usage Patterns (\Cref{sec:usage})}} \\ 
    Viewing time & Total inferred duration & Daily mean & H${>}$L$^{*}$ & - & - \\ 
                 &  & Weekly mean & H${>}$L$^{*}$ & - & - \\ 

    \cmidrule{2-6} 
    
    Session duration & Total viewing time within a session & Mean & - & - & - \\
    Session size     & Total number of videos within a session & Mean & - & - & M${<}$L$^{*}$  \\ 
    Session gap      & Temporal gap between the last video of the previous session and the first video within the subsequent session & Mean & H${<}$L$^{*}$ & - & M${<}$L$^{*}$  \\
    Long session     & Sessions with duration longer than 15 minutes & Ratio & H${>}$L$^{**}$ & - & M${>}$L$^{*}$\\
                     & Sessions with duration longer than 30 minutes & Ratio & H${>}$L$^{*}$ & - & - \\
                     % & Ratio of sessions with duration longer than 45 minutes over all sessions & Ratio \\
    \cmidrule{2-6} 
    
    Engagement & Videos watching till the end & Ratio & - & - & - \\
               & Videos receiving likes or shares or favors & Ratio & - & - & - \\

    \cmidrule{2-6} 
    
    In-net videos        & Videos viewed from followers over all videos & Ratio & - & - & - \\
    Profile-based videos & Videos viewed within a profile over all videos & Ratio & - & - & - \\ \midrule
    
    & \multicolumn{5}{c}{\textbf{Content Patterns (\Cref{sec:content})}} \\ 
    Topic Difference & Difference between topics of all the videos and videos watched till the end & $L_2$ Distance & H${<}$L$^{*}$ & - & M${<}$L$^{*}$  \\ 
                   & Difference between topics of all the videos and videos engaged & $L_2$ Distance & H${<}$L$^{*}$ & - & M${<}$L$^{*}$  \\ 
                   & Difference between topics of videos watched till the end and videos engaged & $L_2$ Distance & H${<}$L$^{*}$ & - & M${<}$L$^{*}$  \\ 

    \cmidrule{2-6} 
    
    Sentiment & Videos with negative sentiments & Daily mean & H${<}$L$^{**}$ & - & - \\ 
              &   & Weekly mean & H${<}$L$^{**}$ & - & - \\ 
              & Videos with positive sentiments & Daily mean & H${>}$L$^{*}$ & - & M${>}$L$^{*}$ \\ 
              &  & Weekly mean & H${>}$L$^{*}$ & - & M${>}$L$^{**}$ \\
    
    \bottomrule
    \end{tabular}
    \label{tab:significance}
    \caption{Summary of metrics used for characterizing TikTok usage and content patterns across addiction groups. Significance is measured by a one-sided Student's t-test. $^{**}: p<0.01$. $^{*}: p<0.05$. }
\end{table*}

==> tab-latex/contigency.tex <==
\begin{table}[h]
    \centering
    \small
    \subfloat[Multi-label classification]{
    \begin{tabular}{cccc}
    \toprule
       \multirow{2}{*}{True} &  \multicolumn{3}{c}{Prediction}  \\
        \cmidrule(lr){2-4}
        & LLA & MLA & HLA \\
        \midrule
       LLA & 1 & 1 & 1 \\
       MLA & 0 & 2 & 2 \\
       HLA & 1 & 0 & 4 \\
    \bottomrule
    \end{tabular}
    }
    \subfloat[Binary classification]{
    \begin{tabular}{ccc}
    \toprule
       \multirow{2}{*}{True} &  \multicolumn{2}{c}{Prediction}  \\
        \cmidrule(lr){2-3}
        & L/MLA & HLA \\
        \midrule
       L/MLA & 4 & 3 \\
       HLA & 1 & 4  \\
    \bottomrule
    \end{tabular}
    }
    \caption{Contigency table for Logistic Regression.}
    \label{tab:contigency-multi}
\end{table}


==> tab-latex/topic-example.tex <==
% \begin{table}[ht]
%     \centering
%     \small
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{lrr}
%     \toprule
%     Topic & Output & Size \\
%     \midrule
%     Cooking & garlic\\_tsp\\_pasta\\_recipe & \num{25592} \\
%     Fashion & fashiontiktok\\_outfitinspo\\_fashion\\_outfit & \num{17407} \\
%     Music & guitar\\_newmusic\\_guitartok\\_song & \num{11590} \\
%     Emotion & mad\\_happen\\_tody\\_wrong & \num{11277} \\
%     Makeup & skincare\\_acne\\_makeup\\_skin & \num{10796} \\
%     Dog & puppy\\_dogsoftiktok\\_dogs\\_dogtok & \num{10399} \\
%     Car & carsoftiktok\\_cars\\_porsche\\_cartok & \num{9070} \\
%     Cat & cats\\_catsoftiktok\\_kitten\\_cattok & \num{8714} \\
%     Hair & hairtok\\_hair\\_hairstyle\\_haircut & \num{7596} \\
%     Relationship & hes\\_guy\\_couplecomedy\\_bf & \num{7587} \\
%     Comedy & pluh\\_standupcomedy\\_standup\\_comedian & \num{7503} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Top 10 largest topics.}
%     \label{tab:top-topic}
% \end{table}



% \begin{table*}[ht]
%     \centering
%     \footnotesize
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabularx}{2\columnwidth}{r ll ll ll}
%     \toprule
%          & \multicolumn{2}{c}{All topics} &  \multicolumn{2}{c}{Till end} &  \multicolumn{2}{c}{Interacted} \\
%          \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
%         & Output & Size & Output & Size & Output & Size \\
%        \midrule
% \multirow{5}{*}{HLA} & Food (garlic, tsp, pasta, recipe) & \num{ 23742 } & Food (garlic, tsp, pasta, recipe) & \num{ 19556 } & Food (garlic, tsp, pasta, recipe) & \num{ 1264 } \\
% &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 14921 } &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 11472 } & Cat (cats, catsoftiktok, kitten, cattok) & \num{ 1170 } \\
% & Makeup (skincare, acne, makeup, skin) & \num{ 13583 } & Makeup (skincare, acne, makeup, skin) & \num{ 11015 } & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 708 } \\
% & Cat (cats, catsoftiktok, kitten, cattok) & \num{ 9645 } & Cat (cats, catsoftiktok, kitten, cattok) & \num{ 6687 } & christiantiktok\_jesus\_christian\_bible & \num{ 637 } \\
% & mad\_happen\_tody\_wrong & \num{ 9140 } & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 6624 } & Music (guitar, newmusic, guitartok, song) & \num{ 618 } \\
% \midrule
% \multirow{5}{*}{MLA} & Food (garlic, tsp, pasta, recipe) & \num{ 16773 } & Food (garlic, tsp, pasta, recipe) & \num{ 14238 } & Cat (cats, catsoftiktok, kitten, cattok) & \num{ 1197 } \\
% &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 7596 } &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 6146 } & Food (garlic, tsp, pasta, recipe) & \num{ 962 } \\
% & Cat (cats, catsoftiktok, kitten, cattok) & \num{ 5959 } & Makeup (skincare, acne, makeup, skin) & \num{ 5031 } & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 918 } \\
% & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 5949 } & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 4569 } & mad\_happen\_tody\_wrong & \num{ 411 } \\
% & 1989taylorsversion\_taylorsversion\_taylornation\_reputationtaylorsversion & \num{ 5927 } & 1989taylorsversion\_taylorsversion\_taylornation\_reputationtaylorsversion & \num{ 4485 } & Relationship (dating, datingadvice, marriedlife, marriage & \num{ 377 } \\
% \midrule
% \multirow{5}{*}{LLA} & Food (garlic, tsp, pasta, recipe) & \num{ 8392 } & Food (garlic, tsp, pasta, recipe) & \num{ 7178 } & Food (garlic, tsp, pasta, recipe) & \num{ 324 } \\
% & Car (carsoftiktok, cars, porsche, cartok) & \num{ 7737 } & Car (carsoftiktok, cars, porsche, cartok) & \num{ 5696 } & 추천\_\_\_ & \num{ 323 } \\
% & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 6681 } & Dog (puppy, dogsoftiktok, dogs, dogtok) & \num{ 5398 } & gay\_lgbt\_lesbian\_lgbtq & \num{ 300 } \\
% &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 6424 } &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & \num{ 5009 } & Car (carsoftiktok, cars, porsche, cartok) & \num{ 283 } \\
% & Music (guitar, newmusic, guitartok, song) & \num{ 4880 } & Music (guitar, newmusic, guitartok, song) & \num{ 3803 } & & Music (guitar, newmusic, guitartok, song) & Music (guitar, newmusic, guitartok, song) & Celebrity (karina, aespa, overthehorizon, sjfjxx)  \\ & \num{ 280 } \\
%     \bottomrule
%     \end{tabularx}
%     \caption{Top 10 largest topics.}
%     \label{tab:top-topic}
% \end{table*}



\begin{table*}[ht]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
    \begin{tabularx}{2.2\columnwidth}{r XXX}
    \toprule
         & All the videos &  Watch till the end &  Interacted \\
         % \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
\midrule
\multirow{5}{*}{HLA} & Food (garlic, tsp, pasta, recipe) & Food (garlic, tsp, pasta, recipe) & Food (garlic, tsp, pasta, recipe)  \\
&Fashion (fashiontiktok, outfitinspo, fashion, outfit) &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & Cat (cats, catsoftiktok, kitten, cattok)  \\
& Makeup (skincare, acne, makeup, skin) & Makeup (skincare, acne, makeup, skin) & Dog (puppy, dogsoftiktok, dogs, dogtok)  \\
& Cat (cats, catsoftiktok, kitten, cattok) & Cat (cats, catsoftiktok, kitten, cattok) & Religion (christiantiktok, jesus, christian, bible)  \\
& Emotion (mad, happen, tody, wrong) & Dog (puppy, dogsoftiktok, dogs, dogtok) & Music (guitar, newmusic, guitartok, song)  \\
\midrule
\multirow{5}{*}{MLA} & Food (garlic, tsp, pasta, recipe) & Food (garlic, tsp, pasta, recipe) & Cat (cats, catsoftiktok, kitten, cattok)  \\
&Fashion (fashiontiktok, outfitinspo, fashion, outfit) &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & Food (garlic, tsp, pasta, recipe)  \\
& Cat (cats, catsoftiktok, kitten, cattok) & Makeup (skincare, acne, makeup, skin) & Dog (puppy, dogsoftiktok, dogs, dogtok)  \\
& Dog (puppy, dogsoftiktok, dogs, dogtok) & Dog (puppy, dogsoftiktok, dogs, dogtok) & Emotion (mad, happen, tody, wrong)  \\
& Celebrity (1989taylorsversion, taylorsversion, taylornation, reputationtaylorsversion) & Celebrity (1989taylorsversion, taylorsversion, taylornation, reputationtaylorsversion) & Relationship (dating, datingadvice, marriedlife, marriage)  \\
\midrule
\multirow{5}{*}{LLA} & Food (garlic, tsp, pasta, recipe) & Food (garlic, tsp, pasta, recipe) & Food (garlic, tsp, pasta, recipe)  \\
& Car (carsoftiktok, cars, porsche, cartok) & Car (carsoftiktok, cars, porsche, cartok) & suggestion  \\
& Dog (puppy, dogsoftiktok, dogs, dogtok) & Dog (puppy, dogsoftiktok, dogs, dogtok) & LGBTQ (gay, lgbt, lesbian, lgbtq)  \\
&Fashion (fashiontiktok, outfitinspo, fashion, outfit) &Fashion (fashiontiktok, outfitinspo, fashion, outfit) & Car (carsoftiktok, cars, porsche, cartok)  \\
& Music (guitar, newmusic, guitartok, song) & Music (guitar, newmusic, guitartok, song) & Celebrity (karina, aespa, overthehorizon, sjfjxx)  \\
\bottomrule
    \end{tabularx}
    \caption{Top 5 largest topics for all the videos, videos watched till the end and videos interacted.}
    \label{tab:top-topic}
\end{table*}

